TelecomRAG: Taming Telecom Standards with Retrieval Augmented Generation and LLMs

Large Language Models (LLMs) have immense potential to transform the telecommunications industry. They could help professionals understand complex standards, generate code, and accelerate development. However, traditional LLMs struggle with the precision and source verification essential for telecom work. To address this, specialized LLM-based solutions tailored to telecommunication standards are needed. Retrieval-augmented generation (RAG) offers a way to create precise, fact-based answers. This paper proposes TelecomRAG, a framework for a Telecommunication Standards Assistant that provides accurate, detailed, and verifiable responses. Our implementation, using a knowledge base built from 3GPP Release 16 and Release 18 specification documents, demonstrates how this assistant surpasses generic LLMs, offering superior accuracy, technical depth, and verifiability, and thus significant value to the telecommunications field.

==> evaluation.tex <==
\section{Implementation and Evaluation}\label{sec:implementation-and-evaluation}

In the following, we present our implementation of the above design (Section \ref{sec:implementation}) and then, using an example query, we compare our implementation against vanilla chat assistants commonly used today (Section \ref{sec:evaluation}).

%@Girma, Can you revise this? It is important to mention the actual APIs used, the LLM model, version, etc., how you built the graphical interface, the things you implemented with \texttt{Langchain}, etc.
\subsection{Implementation}\label{sec:implementation}

 Our RAG-based LLM for Telecommunication Standards implementation is mostly founded on \texttt{Langchain}~\cite{topsakal2023creating}, a framework that provides an array of built-in wrappers and utilities designed to extract reasoning capabilities from language models. We next explain our implementation of the main two stages of our design.

\textbf{Telecom Knowledge Base (Offline stage).}
Prior to using the system, we need to create a knowledge base. To build a knowledge base for telecommunication standards specialization, we gathered the complete set of 3GPP release-16 and release-18 standard specification documents. These documents are in various formats (PDF, TXT, DOCX, DOC), which can be readily processed by the \texttt{DirectoryLoader} method from the \texttt{Langchain.document\_loaders} library, along with custom functions for progress tracking, multi-threading, and error handling (e.g., corrupted file formats).

The extracted data is then prepared for chunking, cleaning, and eventually, creating a database of \emph{embeddings}, i.e., numerical vector representations of text passages in a latent semantic space.  Effective chunking is crucial for capturing context within this space.  Overly short chunks provide insufficient information, while excessively long passages hinder the creation of a rich semantic space and may exceed the LLM's context window limit. To balance these factors, we divided the data into passages of 4000 words with a 100-word overlap between consecutive chunks using the \texttt{CharacterTextSplitter} method from \texttt{Langchain.text\_splitter}. For every passage, we then generated an embedding using  OpenAI's own embedding service via the \texttt{Langchain.embeddings.openai} library. Although OpenAI's embedding model is not publicly disclosed, it is widely assumed that it is based on a transformer architecture. After all the text chunks are encoded, we store them in a \emph{vector store} using \texttt{Chroma}, an AI-native vector database from \texttt{Langchain.vectorstores}.  


\textbf{Document Retrieval Chain and Presentation (Online stage).}
This process establishes a conversational question-answering pipeline leveraging techniques from information retrieval and natural language processing.
We implement this pipeline with the \texttt{ConversationalRetrievalChain} method from \texttt{Langchain.chains} library, which integrates an LLM, \texttt{gpt-4-1106-preview} from OpenAI in our case, and the vector store we created earlier. 

When presented with a new question and conversational context, the chain first ensures contextually-grounded understanding. To this end, it explicitly provides conversation history as input, influencing both the information retrieval stage and the final response generation by the LLM. Then, it may employ a standalone question reformulation step, where the current question is rephrased in light of the chat history to create an optimal query for the retrieval system. This step clarifies potential ambiguities or references from previous questions. Further, the chain leverages the inherent ability of large language models to process and track conversational context,  feeding the chat history directly into the LLM.

Second, the chain transforms the question for optimal retrieval by encoding the adjusted input using the same encoder used for the vector store, i.e., OpenAI's embedding service. This ensures semantic consistency as the input (reformulated) question is projected into the same semantic space as the embeddings stored in the vector store, which allows for simple geometry-based solutions to match the semantic information in the query with that in the knowledge base. 

Third, the chain performs a semantic search within the vector store, where embeddings represent text passages from 3GPP standard documents as mentioned before. To this end, the chain compares the encoded query and the items  in the vector store using \emph{cosine similarity} to identify the embeddings most semantically related to the query. Cosine similarity is a computationally-cheap solution that has proven good performance in this type of applications because it cares primarily about the angle between vectors (embeddings). This means it naturally picks up on the overall ``direction'' of meaning within the text, regardless of the length of the text. This is crucial since two pieces of text can convey the same meaning using different wordings and sentence lengths. Based on this similarity metric, matching passages are retrieved along with their source documents. Once a similarity score is assigned to every pair of input-base embeddings, a standard K-nearest neighbors (KNN) algorithm is employed to find the K most similar embeddings. We use a default value of $K=4$.

Finally, the LLM integrates this information with the conversational history, generating a response that not only aims to answer the question but also demonstrates awareness of the broader dialog and cites its information sources. This pipeline is conveniently wrapped up into an user-friendly web interface using \texttt{Gradio} that resembles that of conventional AI chatbots such as \texttt{Gemini} or \texttt{ChatGPT}, as shown in Fig.~\ref{fig:telecomllm-nle}.

%\textbf{Interface for Question and Answer.} 
%The gr.Interface function from the gradio library is used to create a user-friendly interface for the chatbot. This interface includes text boxes for user input, bot responses, and chat history display. A custom function, handle\_user\_input, processes user messages through the QA chain (\texttt{Langchain}) and updates the chat history. This function is key to the interactive nature of the chatbot. A chat history is also implemented to keep track of the conversation context. 

\begin{comment}
\begin{itemize}
    \item The method to create the chunks of the documents. Fixed length? Algorithm? 
    - The method used is text splitting and token splitting, but eventually text splitting gave better results hence latest version is based on text splitting. 
    -Yes it is a fixed length chunks of 500 and overlap of 25. 
    - The initial embeddings might be based on techniques like Word2Vec, GloVe, or could be learned from scratch by the gpt model, this is not disclosed in OpeAIEmbeddings documentation. 
    \ja{Can you be more specific? how does the text/token splitting work? any reference to a paper or to a known algorithm? If the algorithm is very simple we can just explain it. } 
    You just need to define the chunk length and overlap length then it is upto the GPT model to chunk the documents and create the indexes. 
    
    \item Method to vectorize the chunks. Do you use Dense Passage Retrieval (DPR) \cite{dpr}? (No we are not at least for this version, but the Lanchain retriver might have some better approaches to retrive documents). \ja{Then what is the vectorization method?}
    The vectorization process in OpenAI's embeddings, such as those generated by models like GPT-4, involves transforming text into numerical vectors that represent the semantic and syntactic information contained in the text. 
    S
    
    \item How do you initialize the weights of the encoder? (there are recommended values, depending how much the base LLM you want it to be involved in the Query encoding,  you can set the temperature from 0 to 1, and conversational history may also play a role as part of the question encoding) 
    
    \ja{I didn't know the base LLM was involved in the encoding... My understanding was that the base LLM is not involved in anything related to encoding.}
    
    \item I guess none of the encoders are fine-tuned later, right? (that is right, but you can use templates to create better prompts)
    - We are using the Conversational Retrieval Chain. 
    - 

    \item How do you implement the document search? Maximum Inner Product Search (MIPS)?
        - The base retriver uses cosine similarity but you can also choose other approaches.
        \ja{Good, but the cosine similarity is the affinity metric. My question is regarding the search algorithm (if any).}

    \item How many chunks do you select? Only the best one / top-k?

    %max_input_size = 4096
    %num_outputs = 512
    %max_chunk_overlap = 20
    %chunk_size_limit = 600

    %you can also choose k, to fix the maximum number of similar documents you want (like setting a treshold)
    \ja{Can you clarify the meaning of these parameters?}

    \item How do you generate the input to the LLM (format of the documents + query)? Iterations over the response?

    - We have a function that handle user input and format's the question into a query for the LLM by combining it with existing "chat history", to maintain context. The LLm is used in conjunction with the retriever which provide the relevant documents and chunks from the vectorstore database. 
    \ja{How does this function work? how the query, the chat history and the retrieved documents are combined?}
    

    \item Is there any memory among consecutive queries? Or are they independent? 
    - yes if you don't want that i also implemented clear chat history and memory will not be considered.
    \ja{Good, it is better to have the option of history.}

    \item Any extra detail I am missing?
    - not really :) 
\end{itemize}
\end{comment}




\subsection{Evaluation}\label{sec:evaluation}
\begin{table*}

\caption{ECN Failure Indication data from actual 3GPP document }
\label{table:groundtruth}
\begin{tabular}{|l|l|l|l|l|}

\hline
\textbf{Procedure} &
  \textbf{Initiated} &
  \textbf{Information element name} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Information \\ element \\ required\end{tabular}} &
  \textbf{Information element description} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ECN Failure \\ Indication\end{tabular}} &
  \multirow{2}{*}{IMS-AGW} &
  Context &
  M &
  \begin{tabular}[c]{@{}l@{}}This information element indicates \\ the context for the bearer termination.\end{tabular} \\ \cline{3-5} 
 &
   &
  Bearer Termination &
  M &
  \begin{tabular}[c]{@{}l@{}}This information element indicates the \\ bearer termination for which the ECN\\  failure is reported.\end{tabular} \\ \cline{2-5} 
 &
  \multirow{3}{*}{IMS-ALG} &
  ECN Error Indication &
  M &
  \begin{tabular}[c]{@{}l@{}}This information element indicates\\  an ECN failure event.\end{tabular} \\ \cline{1-1} \cline{3-5} 
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}ECN Failure \\ Indication Ack\end{tabular}} &
   &
  Context &
  M &
  \begin{tabular}[c]{@{}l@{}}This information element indicates the \\ context where the command was executed.\end{tabular} \\ \cline{3-5} 
 &
   &
  Bearer Termination &
  M &
  \begin{tabular}[c]{@{}l@{}}This information element indicates the \\ bearer termination where the command \\ was executed.\end{tabular} \\ \hline
  
\end{tabular}
\end{table*}
%goals of the evaluation,
%relevance of the evaluation 
%Methdology of the valuation 
%

%\subsection{RAG Pipeline for Telecommunications Standards}
%Methodology for evaluation
% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.98\textwidth]{figs/pipeline.pdf}
%     \caption{Retrieval-Augmented Generation Pipeline for Mobile Communication Standards }
%     \label{fig:rag_pipeline}
% \end{figure*}


% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.98\textwidth]{figs/evaluation_methodlogy2.pdf}
%     \caption{Evaluation methodology}
%     \label{fig:evaluation_methodology}
% \end{figure*}
% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.98\textwidth]{figs/llm4telcoevaluation.pdf}
%     \caption{Example evaluation}
%     \label{fig:evaluation}
% \end{figure*}

%Auto fix of codes based on log analysis

%For the evaluation :

% Prepare 10 to 15 questions 
% Get answers from TlecomGPT, ChatGPT and Telcopilot
% Present it in an excel file in a random fascion  and share it with experts to rate the answer 
% accourding to accuracy, verbosity, clarity etc 

% Report the rating in a bar plot 

% x-axis TelecomGPT, ChatGPT and Telcopilot 
% y-axis Accuracy, Clarity, Correctness, etc 

This section presents the evaluation methodology used and discusses the corresponding results. To gauge our system's performance, we presented a 3GPP-specific question, grounded in the truth presented in Table \ref{table:groundtruth}, to our model and to three distinct AI models: Gemini from Google, TelecomGPT—a third-party application built on ChatGPT—and ChatGPT-4. We then compared the performance of these models based on their responses. 
 Our comparative analysis focused on several key metrics, including the relevance, accuracy, completeness of information, reference to source documents, and the overall coherence and clarity of each generated answer according to the ground truth data. As depicted in Figure \ref{fig:evaluation_result}, for the same question based on the ground truth table the different models have different answers. 


\begin{table*} 
\caption{What are the information elements included in the ``ECN Failure Indication'', and how are they defined?}
\footnotesize
\label{tab:evaluation} 
\begin{tabular}{c|p{17cm}>{\arraybackslash}m{18cm}} 
\hline
\rotatebox[origin=r]{90}{\textbf{ChatGPT 4}} & The ``ECN Failure Indication'' is a term that is typically associated with network protocols, specifically with mechanisms that deal with congestion control. ECN stands for Explicit Congestion Notification. This feature enables network nodes to notify each other about network congestion without dropping packets. However, the specific term ``ECN Failure Indication'' isn't standard, and you may be referring to situations where ECN signaling fails or is not properly communicated between network entities. Here's a detailed look at the typical elements related to ECN, which might be relevant to a failure scenario:
\begin{enumerate}
\item	\textbf{ECN-Capable Transport (ECT)} - This is a codepoint in the IP header that indicates that the end-points of the TCP connection are ECN-capable, meaning they can both send and receive ECN signals. There are two ECT codepoints, ECT(0) and ECT(1), which serve slightly different purposes but essentially signal ECN capabilities.
\item	\textbf{Congestion Experienced (CE)} - This is another codepoint in the IP header used by routers experiencing congestion to indicate this status to the end-points of the transmission. When a packet marked with an ECT codepoint encounters congestion, routers that support ECN can mark these packets as CE instead of dropping them.
\item	\textbf{ECN Echo (ECE)} - This is a flag in the TCP header used to indicate that a segment with the CE codepoint has been received. The receiving end uses this flag to notify the sender about the congestion.
\item	\textbf{Congestion Window Reduced (CWR)} - This flag is set by the sending end to signal to the receiving end that it has received the ECE flag and has reduced its congestion window size accordingly. This is an acknowledgment that the sender is responding to the congestion.
\end{enumerate}
When discussing ``ECN Failure Indication'', it might relate to any anomalies or failures in the signaling process among these elements. Here are a few scenarios where ECN could ``fail'':
\begin{itemize}
\item	\textbf{Unsupported ECN:} If any part of the path between sender and receiver does not support ECN, then the ECN signals (ECT, CE) may not be handled or propagated correctly.
\item	\textbf{Incorrect ECN Implementation:} Bugs or incorrect implementations in routers or end hosts can lead to incorrect ECN behavior, such as failing to set CE flags despite congestion or not reacting to ECE flags.
\item	\textbf{ECN Negotiation Failure:} During the TCP handshake, both sides must agree to use ECN. If there is a failure in this negotiation, ECN will not be used, even if both endpoints support it.
\end{itemize}
Understanding specific ECN failure modes would depend on the context in which ECN is being used (like in specific network architectures or for certain types of traffic) and the specific tools and methods used for diagnosing such failures.  
\\ \hline
\rotatebox[origin=r]{90}{\textbf{Gemini Ultra}} & 
Unfortunately, there isn't a universally defined ``ECN Failure Indication'' with a set list of information elements.  ``ECN'' can refer to different things depending on the context, and the specific details of a failure indication would depend on the particular system or protocol involved.
Here's a breakdown of the possibilities:
\begin{itemize}
\item \textbf{IP Networking:} In the context of Internet Protocol (IP) networking, ECN (Explicit Congestion Notification) is a mechanism for routers to signal congestion to senders. It's unlikely there would be a separate ``ECN Failure Indication''. Issues with ECN functionality might be reported through other mechanisms within the specific routing protocol.
\item	\textbf{Other Fields:} ECN can also stand for Engineering Change Notice or Entry Change Notice in various fields. A failure related to an ECN would likely be specific to the system or process that uses those terms and wouldn't have a standardized format.
\end{itemize}
Here are some ways to get more information:
\begin{itemize}
\item	\textbf{Context Clues:} If you encountered the term ``ECN Failure Indication'' somewhere specific, look for surrounding information that might indicate the context (e.g., manuals, software documentation).
\item	\textbf{System Identification:} If you know the system or protocol where you came across this term, searching for its documentation might reveal details about error reporting mechanisms.
\end{itemize}
If you can provide more context about where you encountered ``ECN Failure Indication'', I might be able to offer more specific guidance.
\\ \hline
\rotatebox[origin=r]{90}{\textbf{TelecomGPT}} & 
The ``ECN Failure Indication'' message in the context of telecommunications and protocols isn't explicitly defined in the documents I have available, such as the SMPP specifications and various telecom-related white papers and presentations. It appears you might be referring to a specific protocol message or error indication that might be part of a broader telecommunications standard or proprietary system not covered in these documents.
If the ``ECN Failure Indication'' you are asking about is related to a specific application, protocol, or vendor-specific implementation, it would be helpful to have more context or details about the system in which this term is used. If it is part of a standard not covered in the documents or discussions I have access to, you may need to consult the specific documentation or standards applicable to that protocol or system. If you can provide more details or clarify the specific protocol or context in which you encountered ``ECN Failure Indication'', I can assist you better. Alternatively, if this is related to a standard or system, the relevant documentation or technical support resources for that system may be the best source for detailed information.
\\ \hline
\rotatebox[origin=r]{90}{\textbf{RAG-based TelecomGPT}} & 
ECN failure indicators in the context of 3GPP standards refer to the mechanisms used to report failure events related to Explicit Congestion Notification (ECN) within the IP Multimedia Subsystem (IMS) architecture, particularly between the IMS Access Media Gateway (IMS-AGW) and the IMS Application Level Gateway (IMS-ALG).
According to the provided context:
\begin{itemize}
\item	The ECN Failure Indication procedure is used to report ECN-related failures as specified in clause 6.2.13.4.
\item	The procedure involves the IMS-AGW initiating the ECN Failure Indication and includes mandatory information elements such as Context, Bearer Termination, and ECN Error Indication.
\item	The Context information element indicates the context for the bearer termination.
\item	The Bearer Termination information element indicates the specific bearer termination for which the ECN failure is being reported.
\item	The ECN Error Indication information element indicates an ECN failure event.
\end{itemize}
The ECN Failure Indication is acknowledged by the IMS-ALG with an ECN Failure Indication Ack, which also includes Context and Bearer Termination information elements.
ECN is a feature that allows network nodes to signal network congestion to endpoints, allowing them to adjust their transmission rates to alleviate congestion. In the context of IMS and 3GPP standards, when the IMS-AGW detects congestion (signaled by ECN-CE marks in IP headers), it is supposed to trigger rate adaptation to manage the congestion. If there is a failure in this process, the ECN Failure Indication procedure is used to report the failure to the relevant entities within the IMS network.

Sources: 23334-g30.docx
\\ \hline
\end{tabular}
\end{table*}

\begin{comment}
\begin{figure*}
    \centering
    % First Row
    \subfloat[Gemini]{%
        \includegraphics[width=0.43\textwidth,height=0.7\textwidth, keepaspectratio]{figs/gemini-google.pdf}
        \label{fig:gemini-google}}
    \hfill
    \subfloat[ChatGPT4]{%
        \includegraphics[width=0.43\textwidth,height=0.7\textwidth, keepaspectratio]{figs/chatgpt4.pdf}
        \label{fig:chatgpt4}}
    % Add some vertical space between rows
    \vspace{1cm}
    % Second Row
    \subfloat[TelecomGPT]{%
        \includegraphics[width=0.43\textwidth,height=0.7\textwidth, keepaspectratio]{figs/telecomgpt.pdf}
        \label{fig:telecomgpt}}
    \hfill
    \subfloat[RAG based Telecom LLM]{%
        \includegraphics[width=0.43\textwidth,height=0.7\textwidth, keepaspectratio]{figs/telecomllm-nle.pdf}
        \label{fig:telecomllm-nle}}
    \caption{Evaluation of our RAG based Telecom LLM with the state of the art LLMs}
    \label{fig:evaluation_result}
\end{figure*}
\end{comment}

==> solution.tex <==
\section{LLM-based Retrieval-Augmented Generation for Telecom Standards}\label{sec:solution}

\subsection{Telecommunication Standards Challenges}



%Intro on the work done by standard experts.
%Why do they need to consult documents or obtain specific information? What kind of information do they need to obtain (e.g., numbers, formulas)? Examples? Explain that this is a knowledge-specific task as the information required is factual.

Telecommunication standards experts are pivotal in ensuring industry compliance with global standards. Their work involves the analysis, development, and interpretation of technical specifications from various standardization organizations, such as 3GPP, ETSI, O-RAN, and ITU. The daily responsibilities of these experts include:
\begin{itemize}
    \item Collaborating with engineers, policymakers, and stakeholders to develop and refine standards.
    \item Keeping pace with technological advancements and regulatory needs in telecommunications.
    \item Regularly reviewing and updating documentation such as guidelines, protocols, and technical reports.
\end{itemize}

These professionals must proficiently navigate a range of domain-specific documents across different Standard Development Organizations (SDOs), demanding a specialized skill set focused on consistency and backward compatibility. Their role crucially involves active participation in committees and working groups, leveraging their expertise to guide the future of telecommunication standards. This requires quick and accurate retrieval of information from a vast array of documents to support new contributions.

%\item \ja{Explain that knowledge databases (e.g., 3GPP specifications) change over time. How frequent? Why? Examples?}

 %\item \ja{Why do we need "generation" of text instead of just retrieving information from the documents? We need to elaborate on this as right now it is not clear to me.}
Having expertise in a specific standardization domain is essential, as the competencies required for 3GPP are significantly different from those for ETSI or O-RAN. Furthermore, staying informed about the latest trends and innovations in telecommunications is critical to maintain the relevance and effectiveness of standards in this rapidly evolving field. Knowledge databases in telecommunications, like 3GPP specifications, are dynamic and constantly evolve to adapt to the fast-changing technological landscape and industry needs. These changes occur regularly, such as quarterly updates in the case of 3GPP, or in response to significant technological advancements, regulatory shifts, or emerging market demands.

Given the complexity and range of telecommunications standards, there is an increasing need for leveraging LLMs for text generation and summarization based on factual information. This is especially true for non-domain experts or professionals who specialize in one domain but need insights from another. For example, an expert in 3GPP specifications may find it challenging to grasp the nuances of O-RAN standards without extensive prior knowledge.

In this context, LLM based RAG are invaluable. They can generate concise summaries, simplify technical jargon, and provide comparative insights between different standards. This capability goes beyond mere information retrieval; it transforms dense and complex technical documents into more digestible and comprehensible formats. By doing so, LLM based RAG bridge the knowledge gap between different standardization domains, enabling both experts and non-experts to quickly and clearly understand essential information without delving into the intricacies of each standard.

This approach significantly enhances efficiency and cross-domain collaboration. It allows professionals to rapidly acquaint themselves with the relevant aspects of other telecommunications standards that might influence their work. It also supports informed decision-making, as individuals can draw upon a broader understanding of the field, rather than being constrained by the limits of their immediate expertise.
 


% \begin{itemize}

%     \item \ja{Intro on the work done by standard experts. Why do they need to consult documents or obtain specific information? What kind of information do they need to obtain (e.g., numbers, formulas)? Examples? Explain that this is a knowledge-specific task as the information required is factual.} 
    
%     \item \ja{Explain that knowledge databases (e.g., 3GPP specifications) change over time. How frequent? Why? Examples?}

   
%     \item \ja{Why do we need "generation" of text instead of just retrieving information from the documents? We need to elaborate on this as right now it is not clear to me.}
% % }
%        


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.98\textwidth]{figs/vectorization.pdf}
    \caption{ Vector database creation (only done once, updated with new documents)  }
    \label{fig:Vectorization}
\end{figure*}

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.98\textwidth]{figs/retrieval_2.pdf}
    \caption{ Automatic Multi-Document Retrieval For Telecommunication Standards (executed at every query)  }
    \label{fig:retrieval}
\end{figure*}

\subsection{High-Level Architecture Overview}
The high-level architecture of the LLM-based RAG for telecommunications, as illustrated in Figure \ref{fig:rag_applications_services}, comprises the following key components:

\begin{itemize}
    \item \textbf{Graphical User Interface (GUI):} An adaptable interface designed for diverse user groups, offering a wide range of applications and services for enhanced interaction and experience.
    \item \textbf{Base Large Language Models:} Integration of advanced models like GPT-4, essential for sophisticated language processing, presentation, and generation.
    \item \textbf{Domain-Specific Knowledge Base:} Incorporates  telecommunications documents, such as 3GPP, ETSI, and O-RAN, ensuring industry-specific accuracy and relevance.
    \item \textbf{RAG API Endpoint:} The core component that processes queries and synthesizes responses, leveraging the strengths of both LLMs and the domain-specific knowledge base.
    \item \textbf{User Groups:} Tailored to cater to various users, including solution architects, developers, standards experts, testers, and researchers, to ensure wide applicability.
    \item \textbf{Applications and Services:} Provides a range of services, including question answering, document summarization, network optimization, software code generation, and customer service automation.
\end{itemize}


